On the application of polynomial and NURBS functions for nonlocal response of low dimensional structures

In this paper, the axial vibration of cracked beams, the free flexural vibrations of nanobeams and plates based on Timoshenko beam theory and first-order shear deformable plate theory, respectively, using Eringen's nonlocal elasticity theory is numerically studied. The field variable is approximated by Lagrange polynomials and non-uniform rational B-splines. The influence of the nonlocal parameter, the beam and the plate aspect ratio and the boundary conditions on the natural frequency is numerically studied. The influence of a crack on axial vibration is also studied. The results obtained from this study are found to be in good agreement with those reported in the literature.

==> TimoBeam.tex <==
\subsection{Timoshenko beams}
Numerical results for normalized vibration frequencies are presented in Table\ref{TBT_compari}. It can be seen that the results from different basis functions are comparable to the analytical results~\citep{reddy2007}. It can be inferred that NURBS basis functions requires only fewer degrees of freedom to achieve the same order of accuracy as that of the radial basis functions. Similarly, MLS approximants also require fewer degrees of freedom. \fref{fig:nurbsconvetbt} shows the convergence in case of the NURBS basis function, for mode 1 frequency with decreasing mesh size for various order of the curve. It can be seen that increasing the order of the curve, yields more accurate results. But with decreasing mesh size, all the results approach analytical solution. Note that, the accuracy on a coarse mesh can be improved by increasing the order of the curve. This is an unique advantage in case of the NURBS basis functions. The effect of nonlocal parameter and beam aspect ratio is shown in \frefs{fig:timointlenparam} and (\ref{fig:timoahintlenparam}), respectively. It can be observed that increasing the nonlocal parameter decreases the fundamental frequency. The nonlocal parameter has greater influence on higher modes. The variation of frequency ratio $\Omega_{NL}/\Omega_L$ is shown in \fref{fig:timointlenparam}. For mode 1, the variation is almost linear, but for higher modes, the variation becomes nonlinear. It can be seen from \fref{fig:timoahintlenparam} that increasing the beam aspect ratio increases the frequencies, while increasing the nonlocal parameter decreases the frequency. This is because, increasing the aspect ratio, increases the flexibility of the structure, on the other hand, the nonlocal parameter decreases the local flexibility. The effect of various boundary condition on the fundamental frequency is illustrated in Table \ref{TBT_variousbc}. It can be seen that the effect of nonlocal parameter is to decrease the frequency. The clamped-clamped boundary condition increases the fundamental frequency, while the clamped-free lowers the frequency compared to the simply supported case.

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.6]{./Figures/TBT_mconve}
\caption{Convergence of the first mode with mesh size for various degree of the curve.}
\label{fig:nurbsconvetbt}
\end{figure}

% comparison of fundamental frequency - Timoshenko beam theory 
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Comparison of natural frequencies of simply supported Timoshenko nanobeams. $^\Box$Ref.~\cite{reddy2007}, $^{\dagger\dagger}$1501 global collocation points~\cite{roqueferreira2011}, $^\flat$NURBS basis functions with $p =$ 3 and 82 elements, $^\ast$Lagrange polynomials (100 elements) and $^\sharp$MLS approximants, 100 nodes.}
\begin{tabular}{cclllll}
\hline
$a/h$ & $\mu$ & Analyt- & \multicolumn{4}{c}{Method}\\
\cline{4-7}
&  & ical$^\Box$ & RBF$^{\dagger\dagger}$ & NURBS$^\flat$ & MLS$^\sharp$ & FEM$^\ast$ \\
\hline
\multirow{3}{*}{100} & 0 & 9.8683 & 9.8283 & 9.8680 & 9.8645 & 9.8630 \\
& 1 & 9.4147 & 9.3766 & 9.4144 & 9.4112 & 9.4096 \\
& 5 & 8.0750 & 8.0423 & 8.0748 & 8.0725 & 8.0706\\
\cline{2-7}
\multirow{3}{*}{20} & 0 & 9.8381 & 9.8059 & 9.8281 & 9.8258 & 9.7955\\
& 1 & 9.3858 & 9.3551 & 9.3763 & 9.3742 & 9.3452\\
& 5 & 8.0503 & 8.0239 &  8.0421 & 8.0407 & 8.0154 \\
\cline{2-7}
\multirow{3}{*}{10} & 0 & 9.7454 & 9.7792 &  9.7075 & 9.7034 & 9.5886 \\
& 1 & 9.2973 & 9.3294 & 9.2612 & 9.2538 & 9.1460\\
& 5 & 7.9744 & 8.0014 & 7.9434 & 7.9385 & 7.8445\\
\hline
\end{tabular}
\label{TBT_compari}
\end{table}

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.6]{./Figures/TBT_intLenParam}
\caption{Frequency ratio $(\Omega_{NL}/\Omega_L)$ as a function of nonlocal parameter $\mu$ for $a/h=$ 100 and $L=$ 10 for Timoshenko beam. It can be seen that as the nonlocal parameter increases, the nonlocal effects are prominent. For a fixed nonlocal parameter, the effect of nonlocal parameter on higher frequencies is greater than that for lower modes.}
\label{fig:timointlenparam}
\end{figure}

\begin{figure}[htpb]
\centering
\includegraphics[scale=0.6]{./Figures/TBT_ahIntLenParam}
\caption{Mode 1 non-dimensionalized frequency $(\Omega_{NL})$ as a function of beam aspect ratio $L/h$ for different nonlocal parameters for Timoshenko beam. It can be seen that the effect of nonlocal parameter is to decrease the frequency, whereas, increasing the beam aspect ratio, increases the fundamental frequency}
\label{fig:timoahintlenparam}
\end{figure}

% comparison of fundamental frequency - Timoshenko beam theory 
\begin{table}[htpb]
\centering
\renewcommand\arraystretch{1.5}
\caption{Non-dimensional frequency of Timoshenko beam under various boundary conditions.}
\begin{tabular}{cclll}
\hline
$a/h$ & $\mu$ & \multicolumn{3}{c}{NURBS, $p=$ 3}\\
\cline{3-5}
&  & SS & CC & CF \\
\hline
\multirow{4}{*}{100}& 0 & 9.8680 & 22.3892 & 3.5178\\
& 1 & 9.4144 & 21.1228 & 3.4385 \\
& 2 & 9.0180 & 20.0450 & 3.3639\\
& 5 & 8.0748 & 17.5791 & 3.1646 \\
\cline{2-5}
\multirow{4}{*}{20}& 0 & 9.8281 & 21.9967 & 3.5091\\
& 1 & 9.3763 & 20.7595 & 3.4303 \\
& 2 & 8.9816 & 19.7049 & 3.3561 \\
& 5 & 8.0421 & 17.2877 & 3.1577 \\
\cline{2-5}
\multirow{4}{*}{10}& 0 & 9.7075 & 20.9726 & 3.4884\\
& 1 & 9.2612 & 19.8083 & 3.4107 \\
& 2 & 8.8713 & 18.8124 & 3.3375 \\
& 5 & 7.9434 & 16.5200 & 3.1415 \\
\hline
\end{tabular}
\label{TBT_variousbc}
\end{table}
